Minimum Violation Control Synthesis on Cyber-Physical Systems under Attacks

Cyber-physical systems are conducting increasingly complex tasks, which are often modeled using formal languages such as temporal logic. The system's ability to perform the required tasks can be curtailed by malicious adversaries that mount intelligent attacks. At present, however, synthesis in the presence of such attacks has received limited research attention. In particular, the problem of synthesizing a controller when the required specifications cannot be satisfied completely due to adversarial attacks has not been studied. In this paper, we focus on the minimum violation control synthesis problem under linear temporal logic constraints of a stochastic finite state discrete-time system with the presence of an adversary. A minimum violation control strategy is one that satisfies the most important tasks defined by the user while violating the less important ones. We model the interaction between the controller and adversary using a concurrent Stackelberg game and present a nonlinear programming problem to formulate and solve for the optimal control policy. To reduce the computation effort, we develop a heuristic algorithm that solves the problem efficiently and demonstrate our proposed approach using a numerical case study.

==> formulation_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Problem Formulation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we formulate the problems we investigate in this paper. First, we formulate the minimum violation problem on stochastic system with incompatible specifications. Next, we present the formulation for minimum violation problem on stochastic system with the presence of adversary. We adopt the notions from \cite{raman2012automated} and denote the first problem as unsatisfiability problem while the second problem as unrealizability problem.


We consider a discrete-time stochastic system with dynamics
\begin{equation}\label{eq: dynamics}
x(t+1) = f\left(x(t),u_C(t),u_A(t),\omega(t)\right),~t = 0,1,\cdots,
\end{equation}
where $x(t)\in\mathbb{R}^l$ is the state at time $t$, $u_C(t)\in\mathbb{R}^m$ is the input from the controller, $u_A(t)\in\mathbb{R}^m$ is the attack signal from the adversary and $\omega(t)$ is stochastic disturbance. Here we assume the adversary conducting attacks by tampering control input of system \eqref{eq: dynamics}. Thus the control input of system \eqref{eq: dynamics} $u(t)=u_C(t)+u_A(t)$ for all $t=0,1,\cdots$.

System \eqref{eq: dynamics} is given a set of specifications modeled in co-safe LTL (scLTL) $\Phi=\{\phi_1,\cdots,\phi_n\}$. By satisfying any specification $\phi_i\in\Phi$, system \eqref{eq: dynamics} obtains a reward denoted as $r(\phi_i)$. 
\subsection{Unsatisfiability Problem}

In this subsection, we focus on on the scenario where the specifications cannot be satisfied by system \eqref{eq: dynamics} due to incompatibility of specifications in $\Phi$ and we denote this as unsatisfiability problem. In this case, there is no adversary and thus $u_A(t)=0$ for all $t=0,\cdots$.

Due to the absence of adversary, by abstraction algorithm such as \cite{lahijanian2009probabilistic}, an MDP $\mathcal{M}$ can be constructed for system \eqref{eq: dynamics}. Then the unsatisfiability problem we investigated in this subsection is as follows.

\begin{problem}\label{prob: unsatisfiability problem}
\emph{(Unsatisfiability problem):} Given an MDP $\mathcal{M}$ abstracted from system \eqref{eq: dynamics} and a set of specifications $\Phi=\{\phi_1,\cdots,\phi_n\}$ that cannot be satisfied by system \eqref{eq: dynamics} simultaneously, with each $\phi_i\in\Phi$ associated with a reward function $r(\phi_i)$ for all $\phi_i\in\Phi$, compute a control policy $\mu$ such that the total expected reward obtained by system \eqref{eq: dynamics} is maximized, i.e.,
\begin{equation}\label{eq: reward maximization}
\max_\mu~\mathbb{E} \left\{\sum_{\{\phi_i|\tau_\mu\models\phi_i\}}r(\phi_i)|\mu,s_0\right\},
\end{equation}
where $\tau_\mu$ is the trace induced by policy $\mu$.
\end{problem}

By setting $r(\phi_i)=r$ for all $\phi_i\in\Phi$, \eqref{eq: reward maximization} models the objective that system \eqref{eq: dynamics} is required to satisfy as many specifications as possible. By setting $r(\phi_i)=2^{n-i}$ for all $\phi_i\in\Phi$, system \eqref{eq: dynamics} is required to always satisfy the specification with highest priority.

\subsection{Unrealizability Problem}

In this subsection, we focus on the unrealizability problem where the specifications $\Phi$ cannot be satisfied by system \eqref{eq: dynamics} due to adversary tampering control input by injecting attack signal $u_A(t)$. The adversary's objective is to prevent the system \eqref{eq: dynamics} from satisfying specifications in $\Phi$. We assume the adversary to be strategic player and it can observe the historical behavior of the controller and then play its best response to the control policy $\mu$. However, the controller has no information about the strategy committed by the adversary but the its presence. Moreover, we assume that the controller and adversary take actions simultaneously. Therefore, a concurrent Stackelberg setting is adopted in this paper, and thus randomized control policy is more effective \cite{chatterjee2012survey}.\todo{need citation}

Due to the presence of multiple decision makers (the controller and adversary), system \eqref{eq: dynamics} is abstracted as a stochastic game $\mathcal{G}$ defined in Definition \ref{def: SG}. Moreover, since the objectives of both players (the controller and adversary) are complementary, a zero-sum SG is formulated in the following.
\begin{problem}\label{prob: unrealizability problem}
\emph{(Unrealizability problem):} Given a SG $\mathcal{G}$ abstracted from system \eqref{eq: dynamics} and a set of specifications $\Phi=\{\phi_1,\cdots,\phi_n\}$ that cannot be satisfied by system \eqref{eq: dynamics} simultaneously, with each $\phi_i\in\Phi$ associated with a reward function $r(\phi_i)$ for all $\phi_i\in\Phi$, compute a control policy $\mu$ such that the total expected reward obtained by system \eqref{eq: dynamics} is maximized, i.e.,
\begin{equation}\label{eq: reward maximization}
\max_\mu\min_\lambda~\mathbb{E} \left\{\sum_{\{\phi_i|\tau_{\mu,\lambda}\models\phi_i\}}r(\phi_i)|\mu,\lambda,s_0\right\},
\end{equation}
where $\lambda$ is the policy of adversary and $\tau_{\mu,\lambda}$ is the trace induced by policies $\mu$ and $\lambda$.
\end{problem}

Note that it is sufficient to consider pure strategy of adversary, and thus the search space of SE \cite{conitzer2006computing,filar2012competitive}. Therefore, when investigating Problem \ref{prob: unrealizability problem}, control policy $\mu:S^\ast\times U_C\rightarrow \mathbb{R}$ (resp. adversary policy $\lambda:S^\ast\times U_A\rightarrow \mathbb{R}$) \todo{this definition of probability simplex is incorrect.}is a function specifying the probability distribution over control (resp. attack) actions given historical trajectory $S^\ast$. However, since it is sufficient to consider pure strategy of adversary, we have $\lambda(s_\mathcal{P})\in\{0,1\}$ for all $s_\mathcal{P}$, i.e., $\lambda(\cdot)$ returns a deterministic action at each state \todo{need citation} \cite{conitzer2006computing}.
